Surgical Skill Assessment via Video Semantic Aggregation

Automated video-based assessment of surgical skills is a promising task in assisting young surgical trainees, especially in poor-resource areas. Existing works often resort to a CNN-LSTM joint framework that models long-term relationships by LSTMs on spatially pooled short-term CNN features. However, this practice would inevitably neglect the difference among semantic concepts such as tools, tissues, and background in the spatial dimension, impeding the subsequent temporal relationship modeling. In this paper, we propose a novel skill assessment framework, Video Semantic Aggregation (ViSA), which discovers different semantic parts and aggregates them across spatiotemporal dimensions. The explicit discovery of semantic parts provides an explanatory visualization that helps understand the neural network's decisions. It also enables us to further incorporate auxiliary information such as the kinematic data to improve representation learning and performance. The experiments on two datasets show the competitiveness of ViSA compared to state-of-the-art methods. Source code is available at: bit.ly/MICCAI2022ViSA.

==> 02_related_work.tex <==
\section{Related Work}

\subsection{Surgical Skill Assessment}
The risk of surgical operations raises high requirements on the skill of surgeons. A computer-aided surgical training system that can automatically provide the objective skill assessment and improvement feedback is therefore desired~\cite{jigsaws}. Especially, this supports and improves medical training in resource insufficient countries.

Not only in the community of medical image processing~\cite{surgical_kinematic,surgical_accel,surgical_rmis,surgical_shmm,surgical_predictive,surgical_bilstm,surgical_cnn,surgical_3dcnn,surgical_clearness,surgical_interp,surgical_unified}, the task of surgical skill assessment has also attracted extensive attention in computer vision community as a subtask of action quality assessment~\cite{sd_doughty1,sd_manipulation,sd_doughty2,aqa_jointgraph,aqa_asymmetric}. Existing surgical skill assessment algorithms can be divided into three categories: the first category~\cite{surgical_kinematic,surgical_accel,surgical_rmis,surgical_shmm,surgical_predictive,surgical_bilstm,surgical_cnn} directly uses the kinematics data related to the position and speed of the surgical tools. For example, Fawaz \etal~\cite{surgical_kinematic} made skill-level classification on kinematics data from surgical robots via a 1D CNN. Although the highly motion-related data ensures the sensitivity to the subtle movement of tools, it is only directly available on surgical robots, limiting its applicability. The second group of methods~\cite{sd_doughty1,sd_doughty2,sd_manipulation,surgical_3dcnn,surgical_clearness} focuses on employing only visual information to assess the surgical skills. Doughty \etal~\cite{sd_doughty1,sd_doughty2} proposed to make pairwise skill determination through 2D CNNs. Li \etal~\cite{sd_manipulation} concentrated on finding task-related regions from 2D CNN features and modeling their temporal evolution by LSTMs. Compared to the kinematic data, video data are more abundant, but also contain redundancy besides the visual information related to surgical operations. As the third category, many methods investigate integrating two or more kinds of information related to surgical actions for better performance. Gao \etal~\cite{aqa_asymmetric} combined features from RGB frames and kinematics data. Wang \etal~\cite{surgical_interp} resorted to a multi-task framework to predict skill scores and surgical gestures simultaneously. Liu \etal~\cite{surgical_unified} proposed a multi-path architecture to merge features from four paths: vision, tool, proxy and event. 

Our method aims to achieve better performance in assessing surgical skills from videos by elaborating on aggregating CNN features over spatial and temporal dimensions instead of globally average pooling them.
% Differing from these approaches, our method concentrates on extracting features corresponding to different kinds of semantics from video frames. We then make temporal contextual modeling for them respectively. Meanwhile, our method also enables the incorporation of auxiliary information such as tools kinematics to optimize the semantics separation.

\subsection{Feature Aggregation Learning}
A proper data representation or feature is essential for performance~\cite{representation_define}. Now, it is popular to implicitly learn the representations through deep neural networks in an end-to-end strategy with supervision or rewards at the end. This makes the representations opaque and limits their interpretability~\cite{interpret_survey}. 
Taking one step towards resolving this issue, one type of method aggregates the intermediate representations of CNNs by clustering features to discover regions that have different semantics. They have been utilized to achieve neural network interpretation~\cite{interpret_survey,interpret_tograph,interpret_totree}, semantic segmentation~\cite{featgroup_segment,featgroup_beyondgrids,featgroup_globalreasoning}, object detection~\cite{featgroup_objdetect}, fine-grained recognition~\cite{featgroup_regiongroup}, and action recognition~\cite{featgroup_stgraph,featgroup_globalreasoning,actionvlad}.  Among these works, ones for action recognition focus on a similar task as our ViSA, \ie, understanding videos by modeling the features' relationship in spatiotemporal dimensions. However, Wang and Gupta~\cite{featgroup_stgraph} built graphs upon region features extracted by an extra pre-trained Region Proposal Network (RPN). Chen \etal~\cite{featgroup_globalreasoning} performed the feature grouping and graph-based reasoning on one single 3D-CNN without introducing the long-term contextual modeling. Compared with the aforementioned two methods, we do not need any extra object detector to perform the automatic semantic parts proposal. We also model the long-term relationship of these regional features. ActionVLAD~\cite{actionvlad} made feature aggregation based on the clustered 2D features, which shows a similar framework as ours. However, not limited to the short video, our framework achieves the feature aggregation across both spatial and long-range temporal dimensions. The feature variance in long videos makes the aggregation harder. To solve this challenge, we further introduced existence regularization as well as auxiliary supervision information to optimize the feature grouping. 


==> tex_images/supvis_gui.tex <==
\begin{figure*}[b!]
\centering
\includegraphics[width=\textwidth]{sup_images/camera_calibrate.png}
\caption{The GUI and examples for labeling the kinematics transformation matrix. We sample 3 frames from one video and manually click the center of each clip (marked as the yellow star). The transformation matrix is approximated based on the manually labeled 2D image points and corresponding 3D kinematic points (shown as the title of each frame) by the Direct Linear Transformation algorithm.} 
\label{fig:labelui}
\end{figure*}

==> tex_images/supvis_lstm.tex <==

\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sup_images/LSTM_KT_F1_39.jpg}
         \caption{LSTMs}
         \label{fig:group2}
     \end{subfigure}
     
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sup_images/Part3_KT_F1_39.jpg}
         \caption{BiLSTMs}
         \label{fig:group3}
     \end{subfigure}
     
	 \vspace{1em}
     \caption{Comparison of the assignment maps generated by LSTMs and BiLSTMs.}
% 	 \label{}
\end{figure}

==> tex_images/supvis_tasd.tex <==
\begin{figure*}[t]
	\centering
	\footnotesize
	\renewcommand{\tabcolsep}{1pt}
	\newcommand{\sz}{0.11}
	\newcommand{\hlinevspace}{\hline\vspace{-7pt}}
	\begin{tabular}{cccccccc}
	
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_0.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_4.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_7.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_8.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_12.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_16.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_17.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/img_20.jpg} \\
	
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_0.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_4.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_7.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_8.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_12.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_16.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_17.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_185/assign_20.jpg} \\
	
% 	\hlinevspace \\
	
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_0.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_4.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_7.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_8.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_12.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_16.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_17.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/img_20.jpg} \\
	
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_0.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_4.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_7.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_8.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_12.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_16.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_17.jpg}
% 	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_201/assign_20.jpg} \\
	
    \end{tabular}
	\caption{Visualization of the assignment maps for TASD-2 diving dataset.}
	\label{fig:tasd}
\end{figure*}

==> tex_images/supvis_tasd_r2d.tex <==
\begin{figure*}[t]
	\centering
	\footnotesize
	\renewcommand{\tabcolsep}{2pt}
	\newcommand{\sz}{0.105}
	\renewcommand{\arraystretch}{2}
	\newcommand{\hlinevspace}{\hline\vspace{-7pt}}
	\begin{tabular}{cccccccc}
	
% 	\hlinevspace \\
	
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_0.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_3.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_7.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_8.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_12.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_16.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_17.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/img_20.jpg} \\
	
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_0.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_3.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_7.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_8.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_12.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_16.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_17.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D_112/assign_20.jpg} \\
	
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_0.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_3.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_7.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_8.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_12.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_16.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_17.jpg}
	\includegraphics[height=\sz\linewidth]{sup_images/TASD10m_R2D101_112/assign_20.jpg} \\
	
    \end{tabular}
    \vspace{0.5em}
	\caption{Visualization of the assignment maps generated by setting different numbers of semantic groups on the TASD-2 diving dataset.}
	\label{fig:tasd_r2d}
	\vspace{-1em}
\end{figure*}

==> tex_images/vis_gradcam.tex <==

\begin{figure*}[ht]
	\centering
	\footnotesize
	\renewcommand{\tabcolsep}{1pt}
	\renewcommand{\arraystretch}{2}
	\newcommand{\sz}{0.1}
	\newcommand{\hlinevspace}{\hline\vspace{-4pt}}
	\begin{tabular}{cccccccc}
	
    \vspace{-8pt}
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_12.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_14.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_16.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_18.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_20.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_22.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_28.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_frames/img_30.jpg} 
	\put(-302,4){\rotatebox{90}{\scriptsize{Frames}}} 
	\\
% 	\hlinevspace
	
    \vspace{-4pt}
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_12.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_14.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_16.jpg} & 
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_18.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_20.jpg} & 
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_22.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_28.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_GradCAM/exp_30.jpg} 
	\put(-302,0){\rotatebox{90}{\scriptsize{W/O SGM}}}
	\\
	
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_12.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_14.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_16.jpg} & 
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_18.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_20.jpg} & 
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_22.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_28.jpg} &
	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_GradCAM/exp_30.jpg} 
	\put(-302,2){\rotatebox{90}{\scriptsize{W/ SGM}}}
	\\
	
% 	\hfill
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_12.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_14.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_16.jpg} & 
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_18.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_20.jpg} & 
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_22.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_28.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_0part_SG2/exp_30.jpg} 
% 	\put(-360,0){\rotatebox{90}{\#Group = \textbf{3}}} 
% 	\\
	
% 	\hfill
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_12.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_14.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_16.jpg} & 
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_18.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_20.jpg} & 
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_22.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_28.jpg} &
% 	\includegraphics[height=\sz\linewidth]{exp_images/E1_3parts_SG2/exp_30.jpg} 
% 	\put(-360,0){\rotatebox{90}{\#Group = \textbf{3}}} 
% 	\\
	
    \end{tabular}
    % \vspace{-10pt}
	\caption{Post-hoc attribution results generated by Grad-CAM~\cite{gradcam}. Compared with the framework without employing the semantic grouping module (W/O SGM), the full framework (W/ SGM) concentrates more on the task-related regions such as robotic hands as well as discards more unrelated background regions.}
	\label{fig:gradcam}
\end{figure*}

==> tex_images/vis_htmpregu.tex <==

\begin{figure*}[t]
	\centering
	\footnotesize
	\renewcommand{\tabcolsep}{1pt}
	\newcommand{\sz}{0.1}
	\newcommand{\hlinevspace}{\hline\vspace{-4pt}}
% 	\vspace{-0.7em}
	\begin{tabular}{ccccc|ccccc}
	
    \multicolumn{4}{l}{\scriptsize{Frames}} &  &  & \multicolumn{4}{l}{\scriptsize{Heatmaps for Position Supervision}} \\
	
	\vspace{-4pt}
	\includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/frames/img_8.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/frames/img_9.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/frames/img_10.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/frames/img_11.jpg}
	& &
	
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/heatmaps/assign_8.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/heatmaps/assign_9.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/heatmaps/assign_10.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/heatmaps/assign_11.jpg} \\
	
	\multicolumn{4}{l}{\scriptsize{W/O Position Supervision}} &  &  & \multicolumn{4}{l}{\scriptsize{W/ Position Supervision}} \\
	\includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10/assign_8.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10/assign_9.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10/assign_10.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10/assign_11.jpg}
	& &
	
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10+htmpregu20/assign_8.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10+htmpregu20/assign_9.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10+htmpregu20/assign_10.jpg}
	& \includegraphics[height=\sz\linewidth]{vis_results/4Folds_39_SU_D5/shaping10+htmpregu20/assign_11.jpg} \\
	
    \end{tabular}
	\caption{Improved semantic grouping results after leveraging the supervision of robotic hand positions. The green regions become to concentrate on the robotic hands after using the position heatmaps supervision.}
	\label{fig:heatmap_regu}
\end{figure*}

==> tex_images/vis_modules.tex <==

\begin{figure}
     \centering
	 \newcommand{\asz}{0.59\linewidth}
	 \newcommand{\bsz}{0.39\linewidth}
     \begin{subfigure}[b]{\asz}
         \centering
         \includegraphics[width=\textwidth]{images/Group.pdf}
         \caption{}
         \label{fig:group}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\bsz}
         \centering
         \includegraphics[width=\textwidth]{images/Beta_CDF_54.png}
         \caption{}
         \label{fig:beta}
     \end{subfigure}
     \caption{Semantics disentanglement module (left) and the beta distribution for group existence regularization (right).}
\end{figure}


% \begin{figure}
%     \centering
%     \newcommand{\asz}{0.55\linewidth}
%     \newcommand{\bsz}{0.35\linewidth}
%     \begin{tabular}{cc}
%     % \bmvaHangBox{\fbox{\parbox{2.7cm}{~\\[2.8mm]
%     % \rule{0pt}{1ex}\hspace{2.24mm}\includegraphics[width=2.33cm]{images/Group.pdf}\\[-0.1pt]}}}&
%     % \bmvaHangBox{\fbox{\includegraphics[width=7.5cm]{images/Group.pdf}}}&
%     % \bmvaHangBox{\fbox{\includegraphics[width=4.5cm]{images/Beta_CDF_54.png}}}\\
%     \includegraphics[width=\asz]{images/Group.pdf}&
%     \includegraphics[width=\bsz]{images/Beta_CDF_54.png}\\
%     \end{tabular}
%     \vspace{0.2cm}
%     \caption{Semantics disentanglement module (left) and the beta distribution for group existence regularization (right).}
% \end{figure}


==> tex_tables/res_jigsaws_abl.tex <==
\begin{table}[ht]
\centering
\caption{Ablation study on key framework components or argument. We report and compare the Spearman's Rank Correlations by the 4-Fold cross-validation scheme on three tasks.}
%FEM: Feature Extraction Module, SGM: Semantics Grouping Module, TCMM: Temporal Context Modeling Module, \#Group: the number of semantics groups.}
\vspace{0.2cm}
\label{tab:ablation}
\begin{adjustbox}{width=0.5\textwidth}
\small
% \renewcommand{\arraystretch}{1.2}
\newcommand{\csp}{\hskip 0.1in}

\begin{tabular}{@{}c@{\csp}c@{\csp}c@{\csp}c@{\csp}cccc@{}}
\toprule
% \multirow{2}{*}{semantics disentanglement module} & \multirow{2}{*}{group existence regularization} & \multirow{2}{*}{context modeling module} &
\multirow{2}{*}{FEM} &
\multirow{2}{*}{SGM} &
\multirow{2}{*}{TCMM} &
\multirow{2}{*}{\#Group} &
\multicolumn{4}{c}{4-Fold} \\ \cmidrule{5-8}
& & & & KT & NP & SU & Avg. \\
\midrule
R2D-18 & \xmark  & BiLSTMs & - & 0.48 & 0.74 & 0.29 & 0.53 \\
R2D-18 & \cmark  & BiLSTMs & 3 & 0.67 & 0.82 & 0.54 & 0.69 \\

\midrule
R(2+1)D-18   & \xmark  & LSTMs   & - & 0.60 & 0.81 & 0.68 & 0.71 \\
R(2+1)D-18   & \cmark  & LSTMs   & 3 & 0.67 & \textbf{0.89} & 0.75 & 0.79 \\
\midrule
R(2+1)D-18   & \xmark  & BiLSTMs & - & 0.73 & 0.66 & 0.42 & 0.62 \\
R(2+1)D-18   & \cmark  & BiLSTMs & 2 & 0.83 & 0.86 & 0.71 & 0.81 \\
R(2+1)D-18   & \cmark  & BiLSTMs & 4 & 0.82 & 0.85 & \textbf{0.81} & 0.83 \\
R(2+1)D-18   & \cmark  & BiLSTMs & 3 & \textbf{0.84} & 0.86 & 0.79 & \textbf{0.83} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

%%%%%%%%%% 4-fold, 3 tasks %%%%%%%%%%% 
\begin{table}[ht]
\centering
\caption{Ablation study on each key framework component and argument. We report and compare Spearman's Rank Correlations by the 4-Fold cross-validation scheme on three tasks.}
\label{tab:jigsaws_ablation}
\begin{adjustbox}{width=0.7\linewidth}
\small
% \renewcommand{\arraystretch}{1.2}
\newcommand{\csp}{\hskip 0.1in}
        
\begin{tabular}{@{}c@{\csp}c@{\csp}c@{\csp}c@{\csp}cccc@{}}
\toprule
% \multirow{2}{*}{semantics disentanglement module} & \multirow{2}{*}{group existence regularization} & \multirow{2}{*}{context modeling module} &
\multirow{2}{*}{FEM} &
\multirow{2}{*}{SGM} &
\multirow{2}{*}{TCMM} &
\multirow{2}{*}{\#Group} &
\multicolumn{4}{c}{4-Fold} \\ \cmidrule{5-8}
& & & & KT & NP & SU & Avg. \\
\midrule
R2D-18 & \xmark  & BiLSTMs & - & 0.48 & 0.74 & 0.29 & 0.53 \\
R2D-18 & \cmark  & BiLSTMs & 3 & 0.67 & 0.82 & 0.54 & 0.69 \\
        
\midrule
R(2+1)D-18   & \xmark  & LSTMs   & - & 0.60 & 0.81 & 0.68 & 0.71 \\
R(2+1)D-18   & \cmark  & LSTMs   & 3 & 0.67 & \textbf{0.89} & 0.75 & 0.79 \\
\midrule
R(2+1)D-18   & \xmark  & BiLSTMs & - & 0.73 & 0.66 & 0.42 & 0.62 \\
R(2+1)D-18   & \cmark  & BiLSTMs & 2 & 0.83 & 0.86 & 0.71 & 0.81 \\
R(2+1)D-18   & \cmark  & BiLSTMs & 4 & 0.82 & 0.85 & \textbf{0.81} & 0.83 \\
R(2+1)D-18   & \cmark  & BiLSTMs & 3 & \textbf{0.84} & 0.86 & 0.79 & \textbf{0.83} \\
        
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



==> tex_tables/res_tasd_abl.tex <==

\begin{table}[h]
\centering
\caption{Ablation study on each key framework component and argument. We report and compare Spearman's Rank Correlations by the 4-Fold cross-validation scheme on three tasks.}
\vspace{0.5cm}
\label{tab:ablation}
\begin{adjustbox}{width=0.9\textwidth}
\small
% \renewcommand{\arraystretch}{1.2}
\newcommand{\csp}{\hskip 0.2in}

\begin{tabular}{@{}c@{\csp}c@{\csp}c@{\csp}c@{\csp}c@{\csp}cc@{}}
\toprule
% \multirow{2}{*}{semantics disentanglement module} & \multirow{2}{*}{group existence regularization} & \multirow{2}{*}{context modeling module} &
\multirow{2}{*}{FEM} &
\multirow{2}{*}{SDM} &
\multirow{2}{*}{GER} &
\multirow{2}{*}{CMM} &
\multirow{2}{*}{\#Group} &
\multicolumn{2}{c}{Task} \\ \cmidrule{6-7}
& & & & & SyncDiving-3m & SyncDiving-10m \\
\midrule
ResNet-2D-18 & \xmark & \xmark & BiLSTMs & - &   &   \\
ResNet-2D-18 & \cmark & \cmark & BiLSTMs & 3 & 0.910 & 0.948 \\
\midrule
R(2+1)D-18 & \xmark & \xmark & LSTMs   & - &  &  \\
R(2+1)D-18 & \cmark & \cmark & LSTMs   & 3 &  &  \\
\midrule
R(2+1)D-18 & \xmark & \xmark & BiLSTMs & - &  &  \\
R(2+1)D-18 & \cmark & \xmark & BiLSTMs & 3 &  &  \\
R(2+1)D-18 & \cmark & \cmark & BiLSTMs & 2 & 0.975 & 0.948 \\
R(2+1)D-18 & \cmark & \cmark & BiLSTMs & 4 & 0.968 & 0.955 \\
R(2+1)D-18 & \cmark & \cmark & BiLSTMs & 3 & 0.970 & 0.950 \\

\bottomrule
\end{tabular}
\end{adjustbox}


        
\end{table}

==> tex_tables/two_tables.tex <==
\begin{table}[!b]
    % \vspace{-0.5cm}
    \begin{minipage}{.49\linewidth}
        \centering
        \caption{Ablation study on each key framework component and argument. We report and compare Spearman's Rank Correlations by the 4-Fold cross-validation scheme on three tasks.}
        %FEM: Feature Extraction Module, SGM: Semantics Grouping Module, TCMM: Temporal Context Modeling Module, \#Group: the number of semantics groups.}
        \vspace{0.2cm}
        \label{tab:ablation}
        \begin{adjustbox}{width=\textwidth}
        % \small
        % \renewcommand{\arraystretch}{1.2}
        \newcommand{\csp}{\hskip 0.1in}
        
        \begin{tabular}{@{}c@{\csp}c@{\csp}c@{\csp}c@{\csp}cccc@{}}
        \toprule
        % \multirow{2}{*}{semantics disentanglement module} & \multirow{2}{*}{group existence regularization} & \multirow{2}{*}{context modeling module} &
        \multirow{2}{*}{FEM} &
        \multirow{2}{*}{SGM} &
        \multirow{2}{*}{TCMM} &
        \multirow{2}{*}{\#Group} &
        \multicolumn{4}{c}{4-Fold} \\ \cmidrule{5-8}
        & & & & KT & NP & SU & Avg. \\
        \midrule
        R2D-18 & \xmark  & BiLSTMs & - & 0.48 & 0.74 & 0.29 & 0.53 \\
        R2D-18 & \cmark  & BiLSTMs & 3 & 0.67 & 0.82 & 0.54 & 0.69 \\
        
        \midrule
        R(2+1)D-18   & \xmark  & LSTMs   & - & 0.60 & 0.81 & 0.68 & 0.71 \\
        R(2+1)D-18   & \cmark  & LSTMs   & 3 & 0.67 & \textbf{0.89} & 0.75 & 0.79 \\
        \midrule
        R(2+1)D-18   & \xmark  & BiLSTMs & - & 0.73 & 0.66 & 0.42 & 0.62 \\
        R(2+1)D-18   & \cmark  & BiLSTMs & 2 & 0.83 & 0.86 & 0.71 & 0.81 \\
        R(2+1)D-18   & \cmark  & BiLSTMs & 4 & 0.82 & 0.85 & \textbf{0.81} & 0.83 \\
        R(2+1)D-18   & \cmark  & BiLSTMs & 3 & \textbf{0.84} & 0.86 & 0.79 & \textbf{0.83} \\
        
        \bottomrule
        \end{tabular}
        \end{adjustbox}
    \end{minipage}\hfill
    \begin{minipage}{.49\linewidth}
        \centering
        \caption{Quantitative comparison results against baseline methods on TASD-2 for synchronised diving. We report and compare the Spearman's Correlations on the defined validation sets. \textbf{V}: video frames; \textbf{P}: body poses.}
        \vspace{0.2cm}
        \label{tab:tasd}
        \begin{adjustbox}{width=0.98\textwidth}
        \begin{tabular}{@{}llccc@{}}
        \toprule
        \multirow{2}{*}{Input} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Task} \\ 
        \cmidrule{3-5} 
         &  & 3m & 10m & Average \\ 
        \midrule
        
        \multirow{2}{*}{\textbf{V}}
         & C3D-LSTM~\cite{aqa_olympic} & -0.14 & 0.01 & -0.07 \\
         & I3D-SVR~\cite{aqa_asymmetric} & 0.84 & 0.83 & 0.83 \\
        %  & Ours & \textbf{0.97} & \textbf{0.95} & \textbf{0.96} \\
        \midrule
        
        \multirow{3}{*}{\textbf{V}+\textbf{P}}
         & JR-GCN~\cite{aqa_jointgraph} & 0.89 & 0.81 & 0.86 \\
         & AIM (Single-task)~\cite{aqa_asymmetric} & 0.89 & 0.85 & 0.87 \\
         & AIM (Multi-task)~\cite{aqa_asymmetric} & 0.92 & 0.85 & 0.89 \\
        %  & Ours & \textbf{0.98} & \textbf{0.96} & \textbf{0.97} \\
        \midrule
        
        \multirow{1}{*}{\textbf{V}}
         & ViSA (Ours) & \textbf{0.97} & \textbf{0.95} & \textbf{0.96} \\
        
        \bottomrule
        \end{tabular}
        \end{adjustbox}
    \end{minipage} 
\end{table}






